The Open Porous Media Flow Reservoir Simulator

The Open Porous Media (OPM) initiative is a community effort that encourages open innovation and reproducible research for simulation of porous media processes. OPM coordinates collaborative software development, maintains and distributes open-source software and open data sets, and seeks to ensure that these are available under a free license in a long-term perspective. In this paper, we present OPM Flow, which is a reservoir simulator developed for industrial use, as well as some of the individual components used to make OPM Flow. The descriptions apply to the 2019.10 release of OPM.

==> figures/analytic-upscaling.tex <==
\tikzstyle{edge}=[black, thick, draw]
\tikzstyle{arr}=[black, thick, draw, <->]
\begin{tikzpicture}[scale=0.5]
  \draw [edge] (0,0) -- (15,0) -- (15,5) -- (0,5) -- cycle;
  \draw [edge] (0,5) -- (15,5) -- (15,8) -- (0,8)  -- cycle;
  \draw [arr] (0,-0.5) -- (15,-0.5) node[midway, below]{$l$};
  \draw [arr] (-0.5,0) -- (-0.5,5) node[midway, left]{$d_2$};
  \draw [arr] (-0.5,5) -- (-0.5,8) node[midway, left]{$d_1$};

  \node (k2) at (7.5,2.5) {$k_2$};
  \node (k1) at (7.5,6.5) {$k_1$};
\end{tikzpicture}



